Evidence of Twisted flux-tube Emergence in Active Regions

Elongated magnetic polarities are observed during the emergence phase of bipolar active regions (ARs). These extended features, called magnetic tongues, are interpreted as a consequence of the azimuthal component of the magnetic flux in the toroidal flux-tubes that form ARs. We develop a new systematic and user-independent method to identify AR tongues. Our method is based on determining and analyzing the evolution of the AR main polarity inversion line (PIL). The effect of the tongues is quantified by measuring the acute angle [ tau] between the orientation of the PIL and the direction orthogonal to the AR main bipolar axis. We apply a simple model to simulate the emergence of a bipolar AR. This model lets us interpret the effect of magnetic tongues on parameters that characterize ARs ( e.g. the PIL inclination and the tilt angles, and their evolution). In this idealized kinematic emergence model, tau is a monotonically increasing function of the twist and has the same sign as the magnetic helicity. We systematically apply our procedure to a set of bipolar ARs that were observed emerging in line-of-sight magnetograms over eight years. For most of the cases studied, the tongues only have a small influence on the AR tilt angle since tongues have a much lower magnetic flux than the more concentrated main polarities. From the observed evolution of tau, corrected for the temporal evolution of the tilt angle and its final value when the AR is fully emerged, we estimate the average number of turns in the subphotospherically emerging flux-rope. These values for the 41 observed ARs are below unity, except for one. This indicates that subphotospheric flux-ropes typically have a low amount of twist, i.e. highly twisted flux-tubes are rare. Our results demonstrate that the evolution of the PIL is a robust indicator of the presence of tongues and constrains the amount of twist in emerging flux-tubes

==> readme <==
This directory contains an example paper and informations 
for preparing manuscripts for the journal Solar Physics.

-- Sample              
SOLA_example_6.tex       Sample paper 
SOLA_example_6.pdf       output after compilation (LaTeX, BibTeX, LaTeX, LaTeX of SOLA_example_6) 

-- Files included at compilation
fig1a.eps                        Four figures
fig1b.eps
fig1c.eps
fig1d.eps
SOLA_bibliography_example.bib    Bibliography


-- Extra information
SOLA_keyword_list.txt
SOLA_example_labels.tex
SOLA_Instructions_for_authors.txt


-- Formatting files  
spr-sola-addons.sty
spr-mp-sola.bst
spr-mp-sola-cnd.bst


-- Template
template.tex

-- Notifications
* spr-sola-addons option "linksfromyear" is tested with:
	1. texlive/2008 - natbib 8.1,   hyperref v6.78f
	2. texlive/2009 - natbib 8.31,  hyperref v6.79a
	3. texlive/2010 - natbib 8.31a, hyperref v6.81g
     When hyperref is loaded make a hyperlink only from year component 
     of the cite command. It solves the problem of overfull boxes when dvips driver is used.
     It might not work with an older natbib packages.
     Citation style should be an author-year, and the hyperref should be loaded somewhere in preamble.
* spr-sola-addons loads a natbib package. Use "nonatbib" option if you don't want to load it.



Changes
    * 2014.07.30
         * spr-sola-addons.sty: natbib loaded by default
    * 2011.09.19
         * solarphysics.cls and spr-sola-addons.sty: fixed cite links (when bibliography is created without natbib)
    * 2011.09.16
          o spr-mp-sola.bst and spr-mp-sola-cnd.bst: fixed bug: adding letter to the year field (nameyear)
    *2011.08.04
	  o Renewed sola_example_6.tex. 

    *2011.07.29
	  o Removed \vec from sola_example_6.tex. 

    * 2011.03.01
          o spr-sola-addons.sty:
               1. \TODAY_JWL changed to \TODAY@JWL.	
    * 2010.12.17
          o spr-mp-sola.bst and spr-mp-sola-cnd.bst:
    * 2010.10.14
          o spr-sola-addons.sty:
               1. entered option "linksfromyear", which loads a natbib and puts a link on a year citation.
    * 2010.05.13
          o spr-mp-sola.bst and spr-mp-sola-cnd.bst:
    * 2010.01.26
          o spr-sola-addons.sty:
               1. entered option "solaenum", which makes enumerated list with italics-roman numerals and a single right-bracket.
    * 2009.06.16
          o spr-mp-sola.bst and spr-mp-sola-cnd.bst:
               1. minor fixes.
    * 2009.06.05
          o spr-mp-sola.bst and spr-mp-sola-cnd.bst:
               1. added letters to the years (in bibliography), if authors and years are the same.
    * 2009.06.04
          o spr-mp-sola.bst and spr-mp-sola-cnd.bst:
               1. added letters to the volume ("CS-" if publisher = "ASP" and "SP-" if publisher = "ESA")
               2. \doiurl in \textsf font
    * 2009.06.03
          o spr-mp-sola.bst and spr-mp-sola-cnd.bst:
               1. added letters to the \citeauthoryear{}{} year section (if the same year)
               2. not cutting letters from the pages any more
          o solarphysics.cls :
               1. "," taken off from the \inlinecite
    * 2009.06.02
          o spr-mp-sola.bst and spr-mp-sola-cnd.bst:
               1. doi links out to http://dx.doi.org (using with \usepackage{hyperref}])
    * 2008.06.18
          o natbib option added to spr-sola-addons.sty. Use this option to load a natbib package. (\usepackage[optionalrh,natbib]{spr-sola-addons})
    * 2008.04.23
          o journal's style - modified the footer
          o spr-mp-sola.bst
          o spr-mp-sola-cnd.bst
    * 2007.10.09
          o template added, modifications to spr-sola-addons and example file
    * 2007.08.01 spr-mp-sola
    * 2007.07.10 spr-mp-sola
    * 2007.04.16 spr-sola-addons
          o minor amendmends
    * 2007.03.23 sola-support.zip
          o solarphysics.zip, url.sty files added to the package
    * 2007.03.23 spr-sola-addons, template
          o minor amendmends: running author/title, email
    * 2007.02.28 template.tex
          o included into the distribution
    * 2007.02.23 spr-sola-addons
          o sectioning counter format amended
          o urlstyle introduced (sans serif)


